Universal Checkpointing: A Flexible and Efficient Distributed Checkpointing System for Large-Scale DNN Training with Reconfigurable Parallelis

Deep neural network (DNN) training continues to scale rapidly in terms of model size, data volume, and sequence length, to the point where multiple machines are required to fit large models for training. Different distributed and parallel training strategies have been developed to support large-scale DNN training by partitioning the training state across GPUs. However, existing DNN training systems provide very limited support for reconfiguring parallelism strategies in the middle of the training via checkpointing. This limitation arises because distributed checkpoints are tightly coupled to specific model parallelism and hardware configurations, preventing large-scale training jobs from efficiently adapting to hardware failures or resource elasticity. This paper presents Universal Checkpointing (UCP), a novel checkpointing system that enables flexible and efficient DNN training with reconfigurable parallelism. UCP overcomes challenges in existing systems by decoupling checkpoint structure from parallel training strategies and hardware configurations. In addition, we present a pattern-based reconfiguration pipeline that enables automatic, flexible, and efficient mapping of checkpoint state to various parallelism strategies. Evaluation on a range of DNN models, including state-of-the-art dense and sparse LLMs, shows that UCP enables reconfiguration for a broader set of widely used parallelism strategies than existing solutions while adding negligible reconfiguration cost. UCP has been successfully employed in real LLM training workloads, greatly enhancing their flexibility and resilience to dynamic hardware environments.

==> _tmp_terminology.tex <==
\section*{Terminology}

\paragraph{Universal Checkpointing} The method or format of a unified checkpoint we propose.
\paragraph{\UCP} The abbreviation for Universal Checkpointing.
\paragraph{atomic checkpoints} Checkpoint files saved in the UCP format.
\minjia{How about we use \emph{atomic checkpoints} to refer to the actual checkpoints from \UCP?}\xinyucomment{For sure} \minjia{There are places we still use atom checkpoints from previous submission. Need to do a consistent check at the end.}
\paragraph{Metadata of checkpoints} Information such as number of iterations, loss scaler, gradient clipping parameters, etc.
\paragraph{ZeRO-x} Use a hyphen to connect ZeRO and its stage (e.g., ZeRO-1, ZeRO-2, ZeRO-3).
\paragraph{Optimizer states} Components of the optimizer, including momenta and variances.
\paragraph{Parameter} A single layer in an LLM model, including weights and biases.
\minjia{Mostly agree, although a "layer" in LLMs is often more coarse-grained than a parameter. Let's call individual operator in a model as a parameter, e.g., a Linear operator can be defined a parameter. A logical block that performs a set of operations to refine representation is a layer, e.g., a Transformer block is a layer. A layer can be stacked to form deep DLs. A Transformer layer contains two sublayers, MHA and MLP. Each sublayer contains a set of parameters.}

\paragraph{Capitalization}
\begin{itemize}
    \item ZeRO
    \item DeepSpeed
    \item LLaMA
    \item Megatron-LM
    \item BLOOM
\end{itemize}

\minjia{Agreed on all the rest of the terminology definition.}

\paragraph{Reconfigurable parallelism} Let's use reconfigurable parallelism as the feature UCP provides.

\paragraph{Reconfiguration} We will use reconfiguration to primarily refer to the transformation of checkpoint formats. However, it is okay to use reconfiguration and transformation interchangeably. 


==> optimizer_legacy.tex <==
\section{Parallelism Optimizer}

\minjia{Key challenges:}

When the hardware config changes, the parallelism strategy needs to change as well. However, it is non-trivial to identify the best parallel strategy because (1) the search space of parallelism strategy is huge, 3D parallel, ZeRO-1/2/3, SP. (2) The evaluation cost of each strategy is expensive, e.g., UCP conversion and loading is not free. (3) Preemption pattern varies, e.g., at very high preemption rate, the time spent on finding a good target parallelism strategy becomes part of the training cost, and spending too much time on finding a good parallelism strategy may not bring end-to-end training time reduction. 
(4) Compatibility, ZeRO3 is not compatible with PP, and SP (DeepSpeed-Ulysses) is not compatible with TP and PP.

\minjia{Our solution:}

\begin{itemize}
    \item Stage 1: Define the search space, e.g., parallelism strategies as well as additional system knobs that are important, e.g., bucketization size during backpropagation.
    \item Stage 2: Search space pruning. (i) Comparability checks, e.g., zero3 is not compatible with PP. (ii) Memory capacity constraints check, e.g., DP will definitely not fit a model. 
    \item Stage 3: Initialization. We build performance models for 3D parallelism and ZeRO-1/2/3 to find a small subset of promising configurations.
    \item Stage 4: Learning-based optimization. XGBoost + SA optimizer. 
\end{itemize}

\subsection{While-box performance model + black-box ML-based auto-tuning}

Since evaluating of each config is very expensive, we develop a compute/memory/communication analysis model for 4D parallelism + ZeRO1/2/3 to quickly identify a small subset of promising configs to start the search process, i.e., pruning out non-promising configs.

We use linear regression (e.g., XGBoost) + Optimizer (e.g., simulated annealing) to navigate the search space, using the subset of promising configs identified above as a priori to quickly find a good Target. (We may reuse Deepspeed Autotuner but need efforts to enable for UCP). \xinyu{I will look into the Deepspeed Autotuner.} \xinyu{If the preemption rate is high, we can randomly select one strategy from the small subset, no need to do the profiling-based search.}

\minjia{TODO: Check ranking-based performance model Tunji suggested. If we have a sufficiently good perf model, then we may not need heavy tuning.}

\subsection{Preemption-Aware Scheduling}

In practice, preemption pattern varies, e.g., the preemption pattern of spot instances varies across regions, seasonality, diurnal. Therefore, there is a trade-off between the time spent on finding a good target parallelism strategy vs. the actual benefit from using the found target strategy for the subsequent training steps. If preemption rate is low, then it makes more sense to spend some time to search a good strategy, so that all subsequent training steps can benefit. Otherwise, it may make more sense to use an analytic model to select a parallel strategy, which may not be the optimal one but is better than random selection. \xinyu{I like the idea.} 

Assume we know the preemption pattern, that would make the above decision easier.  But in practice, preemption patterns are hard to predict.  Need more thinking here. \xinyu{We might need one model that can learn from the previous trace to predict the preemption pattern (rate).}

\begin{itemize}
    \item Low preemption rate: Invoke more expensive but also more accurate optimizer (stage 4).
    \item High preemption rate: Skip stage 4. 
\end{itemize}


\section{Efficient System Implementations for \UCP Loading, Conversion, and Saving}

Highly optimized \UCP checkpoint conversion/loading mechanism. Parallelism + NVMe + redundancy reduction. 
This helps improve the efficiency of \UCP, and mostly importantly bring down the evaluation cost of a parallelism strategy.

\minjia{Checkpoint saving cost is also crucial for training with preemptive instances. In spot instance, there is often a grace period. However, this grace period is often quite short, e.g., 2 minutes, which may not be sufficient to save distributed checkpoints. If a checkpoint is not saved on time, then all the work that has been done without saving are wasted. So it is actually important to also discuss the checkpoint saving cost.}

\xinyu{One possible solution is to set a small saving interval.}
\xinyu{The UCP's cost savings are consistent with previous practices. To reduce these costs further, we must revise our existing savings strategies.}
\xinyu{It's intriguing to consider how our implementation can manage a grace period. The time required for saving also varies depending on the model size. We can even have different saving strategies to handle different sizes of the models.}
\xinyu{The worst case is that if we cannot save the checkpoint on time, we would have to resume training using checkpoints from the previous save interval, which is less than ideal.}

\begin{itemize}
    \item \UCP loading: This can be the major bottleneck, e.g., as the model size increases, the redundancy for each rank to load the whole model states is going to hurt the \UCP performance and scalability more. 
    \item \UCP conversion: We may make \UCP conversion eager and asynchronous, e.g., by creating a snapshot of the model states in CPU memory and having separate CPU to asynchronously convert \UCP checkpoints. Once the conversion is done, the original Source checkpoints probably need to be evicted to avoid duplicated checkpoints.  
    \item \UCP saving: potential idea includes creating a snapshot of model states in CPU memory and asynchronously saving model checkpoints while overlapping with training compute. The main concern here is that similar idea has been explored in CheckFreq (need to double check), so it is hard to claim novelty. Also, this method is not free, e.g., creating the CPU snapshot slows down training. 
\end{itemize}

\minjia{TODO: Check FastPersistent. Optimizations that we can benefit: 1. Parallel saving/loading. 2. GPUDirect. 3. Pipelined checkpointing. 4. Asynchronous saving, e.g., CPU snapshot.}

==> spacing.tex <==
% \usepackage[skip=2pt]{caption}
\usepackage{setspace}
\usepackage{enumitem}
\usepackage{titlesec}

% \captionsetup[subfloat]{captionskip=1pt}
% \captionsetup[subfloat]{captionskip=1pt}

% % \newtoggle{tech-report}
% % \toggletrue{tech-report}
% % % \togglefalse{tech-report}

% % \iftoggle{tech-report}{%
% % }{
% \renewcommand{\baselinestretch}{1}
% % }

% \setlist{nosep} % Change space between items in a listing.
\setlength{\textfloatsep}{7pt} % Control space after figure and before text. 
% \setlength{\dbltextfloatsep}{2pt}

% \setlength{\intextsep}{2ex} % remove extra space above and below in-line float (reduce space in between figure caption and the text below it)

% \newlength{\sectionbelowskip}
% \newlength{\sectionaboveskip}
% \newlength{\subsectionbelowskip}
% \newlength{\subsectionaboveskip}
% \newlength{\subsubsectionbelowskip}
% \newlength{\subsubsectionaboveskip}
% \newlength{\paragraphaboveskip}
% \newlength{\paragraphbelowskip}

%  Control space before and after table
% \newcommand{\spaceabovetable}{\vspace*{-1em}}
% \newcommand{\spacebelowtable}{\vspace*{-1em}}
% \newcommand{\spaceabovetable}{\vspace*{2em}}
% \newcommand{\spacebelowtable}{\vspace*{2em}}

% \usepackage{titlesec-custom}

% % Avoid starting a new line for subsubsection
% % \makeatletter
% % \renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
% %                                      {-3.25ex\@plus -1ex \@minus -.2ex}%
% %                                      {-1.5ex \@plus -.2ex}% Formerly 1.5ex \@plus .2ex
% %                                      {\normalfont\normalsize\bfseries}}
% % \makeatother

% \titleformat{\subsubsection}[runin]% runin puts it in the same paragraph
%         {\normalfont\normalsize\bfseries}% formatting commands to apply to the whole heading
%         {\thesubsubsection}% the label and number
%         {0.5em}% space between label/number and subsection title
%         {}% formatting commands applied just to subsection title
%         [.]% punctuation or other commands following subsection title
% \titleformat{\subsubsection}
%   {\normalfont\normalsize\bfseries}{\thesubsubsection}{1em}{}
% \titlespacing*{\subsubsection}{0pt}{\subsubsectionaboveskip}{\subsubsectionbelowskip}

% \newcommand{\setvspace}[2]{%
%   #1 = #2
%   \advance #1 by -1\parskip}

% Ever so slightly tighter than defaults:
% \setvspace{\sectionaboveskip}{4pt plus 1pt minus 1pt}
% \setlength{\sectionbelowskip}{2pt plus 1pt minus 1pt}
% \setlength{\subsectionbelowskip}{2pt plus 2pt minus 0pt}
% \setvspace{\subsectionaboveskip}{1pt plus 2pt minus 2pt}
% % \setlength{\subsubsectionbelowskip}{1pt plus 0pt minus 2pt}
% % \setvspace{\subsubsectionaboveskip}{1pt plus 0pt minus 2pt}
% \setvspace{\paragraphaboveskip}{1pt}
% \setvspace{\paragraphbelowskip}{1pt}
% \setvspace{\sectionaboveskip}{1pt plus 4pt minus 2pt}
% \setlength{\sectionbelowskip}{1pt plus 2pt minus 2pt}
% \setvspace{\subsectionaboveskip}{1pt plus 2pt minus 2pt}
% \setlength{\subsectionbelowskip}{0pt plus 2pt minus 2pt}
% \setvspace{\subsubsectionaboveskip}{1pt plus 4pt minus 2pt}
% \setlength{\subsubsectionbelowskip}{1pt plus 4pt minus 2pt}
% \setvspace{\paragraphaboveskip}{1pt}
% \setvspace{\paragraphbelowskip}{1pt}


% % \titlespacing*{\section}{0pt}{\sectionaboveskip}{\sectionbelowskip}
% \titlespacing{\subsection}{0pt}{0pt}{0pt}
% \titlespacing*{\paragraph}{1pt}{\paragraphaboveskip}{*}


\makeatletter % Control space around theorem and lemma
\def\thm@space@setup{%
  \thm@preskip=3pt
  \thm@postskip=\thm@preskip % or whatever, if you don't want them to be equal
}
\makeatother

% % Control space around itemize items
\setlist[itemize]{noitemsep, topsep=0pt}

% control space above and below equation.
\makeatletter
\g@addto@macro\normalsize{%
  \setlength\abovedisplayskip{1pt}
  \setlength\belowdisplayskip{1pt}
  \setlength\abovedisplayshortskip{1pt}
  \setlength\belowdisplayshortskip{1pt}
}
\makeatother

% \makeatletter % Control the space around the proof.
% \renewenvironment{proof}[1][\proofname]{\par
%   \vspace{1pt}% remove the space after the theorem
%   \pushQED{\qed}%
%   \normalfont
%   \topsep0pt \partopsep0pt % no space before
%   \trivlist
%   \item[\hskip\labelsep
%         \itshape
%     #1\@addpunct{.}]\ignorespaces
% }{%
%   \popQED\endtrivlist\@endpefalse
%   \addvspace{3pt plus 3pt} % some space after
% }
% \makeatother 

% \setlength{\itemindent}{0em}

==> tables/compare.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{lccccccc}
\toprule
 & \multicolumn{5}{c}{\bf Multi-Parallel Strategy} & \multirow{2}{*}{\bf Multi-Framework} & \multirow{2}{*}{\bf Multi-Model Arch.} \\
 \cline{2-6}
 & DP~\cite{ddp} & TP~\cite{megatron-lm-v2} & PP~\cite{1f1b} & SP~\cite{sp} & ZeRO~\cite{zero-optimizer} & \\
\midrule
CheckFreq~\cite{checkfreq} & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
Gemini~\cite{gemini} & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
% JIT & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
DCP~\cite{dcp} & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark \\
MCP~\cite{mcp} & \cmark & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark \\
UCP & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark\\
\bottomrule
\end{tabular}
\caption{\new{Flexibility of checkpoint systems with various parallelism strategies, frameworks and model architectures.}}
% \minjia{TODO: Minor. For captions, either we add a "." at the end of all captions or we don't. I usually add "." to all captions. }
% \xinyucomment{Got it. Let's add "." to all captions.}
\label{tab:comparison}
\end{table*}

==> tables/issue.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{lcccc}
\toprule
 & \textbf{DeepSpeed} & \textbf{Megatron-LM} & \textbf{Pytorch-Lightning} & \textbf{Huggingface-Accelerate} \\
\midrule
Change Parallelism Strategies & 11 & TBA & TBA & TBA \\ 
Change the Platform & 11 & TBA & TBA & TBA \\
CPU OOM & 6 & TBA  & TBA & TBA \\
Change the Parameter & 6 & TBA & TBA & TBA \\
Save Partial Checkpoint & 5 & TBA & TBA & TBA\\
\bottomrule
\end{tabular}
\caption{Checkpoint-related issues in four popular DNN training frameworks.}
\label{tab:issue}
\end{table*}
